Large Language Models: A Survey

Large Language Models (LLMs) have drawn a lot of attention due to their strong performance on a wide range of natural language tasks, since the release of ChatGPT in November 2022. LLMs' ability of general-purpose language understanding and generation is acquired by training billions of model's parameters on massive amounts of text data, as predicted by scaling laws \cite{kaplan2020scaling,hoffmann2022training}. The research area of LLMs, while very recent, is evolving rapidly in many different ways. In this paper, we review some of the most prominent LLMs, including three popular LLM families (GPT, LLaMA, PaLM), and discuss their characteristics, contributions and limitations. We also give an overview of techniques developed to build, and augment LLMs. We then survey popular datasets prepared for LLM training, fine-tuning, and evaluation, review widely used LLM evaluation metrics, and compare the performance of several popular LLMs on a set of representative benchmarks. Finally, we conclude the paper by discussing open challenges and future research directions.

==> others/intro-1.tex <==
\section{Introduction}
Language modeling is a long-standing research topic, dating back to in the 1950s with Shannon's application of information theory to human language, where he measured how well simple n-gram language models predict or compress natural language text. 
Since then, statistical language modeling became fundamental to many natural language understanding and generation tasks, ranging from speech recognition, machine translation, to information retrieval \cite{jelinek1998statistical,manning1999foundations,manning2009introduction}.

The recent advances on transformer-based large language models (LLMs), pretrained on Web-scale text corpora, significantly extended the capabilities of language models (LLMs). For example, OpenAI's ChatGPT and GPT-4 can be used not only for natural language processing, but also as general task solvers to power. Microsoft's Co-Pilot systems, for instance, can follow human instructions of complex new tasks performing multi-step reasoning when needed. LLMs are thus becoming the basic building block for the development of general-purpose AI agents or artificial general intelligence (AGI).

As the field of LLMs is moving fast, with new findings, models and techniques being published in a matter of months or weeks \cite{zhao2023survey,zhou2023comprehensive,liu2023pre,dong2022survey,huang2022towards}, AI researchers and practitioners often find it challenging to figure out the best recipes to build LLM-powered AI systems for their tasks. This paper gives a timely survey of the recent advances on LLMs. We hope this survey will prove a valuable and accessible resource for students, researchers and developers.


Statistical language models (SLMs) view text as a sequence of words, and estimate the probability of text as the product of their word probabilities. The dominating form of SLMs are Markov chain models known as the n-gram models, which compute the probability of a word conditioned on its immediate proceeding $n-1$ words. Since word probabilities are estimated using word and n-gram counts collected from text corpora, the model needs to deal with data sparsity (i.e., assigning zero probabilities to unseen words or n-grams) by using \emph{smoothing} where some probability mass of the model is reserved for unseen n-grams \cite{chen1999empirical}. N-gram models are widely used in many NLP systems. However, these models are incomplete in that they cannot fully capture the diversity and variability of natural language due to data sparsity.  



Early neural language models (NLMs) \cite{bengio2000neural,mikolov2010recurrent,graves2013generating} deal with data sparsity by mapping words to low-dimensional continuous vectors (embedding vectors) and predict the next word based on the aggregation of the embedding vectors of its proceeding words using neural networks. The embedding vectors learned by NLMs define a hidden space where the semantic similarity between vectors can be readily computed as their distance. 
This opens the door to computing semantic similarity of any two inputs regardless their forms (e.g., queries vs. documents in Web search \cite{huang2013learning}, sentences in different languages in machine translation \cite{sutskever2014sequence}) or modalities (e.g., image and text in image captioning \cite{fang2015captions}). Early NLMs are task-specific models, in that they are trained on task-specific data and their learned hidden space is task-specific.


\subsection{Brief History of Language Models}
%[Xavier] This section, does not read very "historical" despite the title. I would stress the timeline of when the different LMs appeared. For example: "Statistical Language Models, that started in the 90s...". Also it feels we lack a definition for "Language Model".
Looking at the history of prominent works on language models: Shannon's work \cite{shannon1951prediction} laid out the foundation of mathematical and statistical frameworks for language understanding, however that was not using any neural based modeling. 
In \cite{rumelhart1985learning}, Rumelhart and Hinton presented the early works on distributed word representation.
Another prominent work was the work "finding structure in time" by Elman \cite{elman1990finding}, in which he presented one of the early works on recurrent neural language models.
Later in \cite{mahoney2000fast}, Mahoney proposed a simple neural net architecture, that achieved state of the art performance in data compression, and it seemed to be open source (PAQ project). Although the model was technically more similar to logistic regression, but this was still a great work showing the promise of this approach.

Although all previous works had significant impact in pushing this field forward, "Neural Probabilistic Language Model" \cite{bengio2000neural} by Bengio et al. is sought to be the first good-performing neural language model on a small dataset and with real data (note that Elman's work proposed previously was using synthetic data).
The work by Schwenk et al. \cite{schwenk2006continuous} presented the first applications of these frameworks for machine translation (MT), achieved good results in MT competitions (WMT). However this model  didn't really scale well, as its performance dropped with training corpus size, when compared to n-gram baseline. 

Then in \cite{mikolov2011strategies, rnnlm}, Mikolov released "RNNLM", an open source neural language modeling toolkit, which was one of the first models that actually scaled well with more data, using different tricks. 
This was one of the first neural network based frameworks (which was very surprising back in 2010) that could beat n-gram based models on large datasets (which at that time had hundreds of millions of words). 
This was the first neural based model to report improving performance with data set size (i.e. the bigger the training set, the bigger the gain from the model). This work led to beginning of deep learning revolution in NLP space. Mikolov trained models with billions of parameters on hundreds of millions of words at the time.
RNNLM was also the first model that showed the potential of neural language model for text generation.
\iffalse
Fig \ref{fig:rnnlm} shows the high-level idea of this framework.
\begin{figure}[h]
\begin{center}
    \includegraphics [scale=0.6] {img/rnnlm.png}
\end{center}
  \caption{Feedforward neural network 4-gram model (on the left) and Recurrent
neural network language model (on the right), proposed by Mikolov et al. Courtesy of \cite{mikolov2011strategies}.}
\label{fig:rnnlm}
\end{figure}
\fi

%There were a series of other prominent works later by Tomas Mikolov, Richard Socher, Ronan Collobert, Jason Weston that showed more promising results by using neural language modeling on a wider range of tasks after that
Some of the key factors contributing to the success of these early prominent frameworks includes: creating better and large benchmarks (first being modified PTB), good choice of hyper-parameters, and more computational power (GPUs) which enabled researchers to train bigger and bigger models. 
New architectures (LSTM, GRU, and then Transformers), and techniques (such as new normalization, and attentions) also had good impact on the overall success of these models.


% \subsection{More Recent Language Models and applications}
% [Xsvier] I think we should mention and cite ULMFit https://arxiv.org/abs/1801.06146
Pre-trained language models (PLMs), unlike early NLMs, are task-agnostic. This generality also extends to the learned hidden embedding space. The training and inference of PLMs follows the \emph{pre-training and fine-tuning} paradigm, where language models with recurrent neural networks \cite{peters2018deep} or transformers \cite{devlin2018bert,liu2019roberta,he2020deberta} are pre-trained on Web-scale unlabeled text corpora for general tasks such as word prediction, and then finetuned to specific tasks using small amounts of (labeled) task-specific data. Recent surveys on PLMs include \cite{zhou2023comprehensive, han2021pre,qiu2020pre}. 

\begin{figure*}
\begin{center}
    \includegraphics [scale=0.57] {img/LLMCap.pdf}
\end{center}
  \caption{LLM Capabilities.}
  \label{fig:llm_cap}
\end{figure*}

%[Xavier] I think we should mention Table III as a way to understand what does "large" mean in this context
Large language models (LLMs) mainly refer to transformer-based neural language models \footnote{Recently, several very promising non-transformer LLMs have been proposed, such as the LLMs based on structured state space models \cite{gu2022S4,gu2023mamba}. See Section \ref{sec:LLM_challenges} for more details.} that contain tens to hundreds of billions of parameters which are pre-trained on massive text data, such as PaLM \cite{chowdhery2022palm}, LLaMA \cite{touvron2023llama}, and GPT-4 \cite{gpt4}, as summarized in Table III.  
Compared to PLMs, LLMs are not only much larger in model size, but also exhibit stronger language understanding and generation abilities, and more importantly, emergent abilities that are not present in smaller-scale language models. As illustrated in Fig.~\ref{fig:llm_cap}, these emergent abilities include (1) in-context learning, where LLMs learn a new task from a small set of examples presented in the prompt at inference time, (2) instruction following, where LLMs, after instruction tuning, can follow the instructions for new types of tasks without using explicit examples, and (3) multi-step reasoning, where LLMs can solve a complex task by breaking down that task into intermediate reasoning steps as demonstrated in the chain-of-thought prompt \cite{Wei2022COT}. 
LLMs can also be augmented by using external knowledge and tools \cite{mialon2023augmented,peng2023check} so that they can effectively interact with users and environment \cite{yao2022react}, and continually improve itself using feedback data collected through interactions (e.g. via reinforcement learning with human feedback (RLHF)). We will look at how LLMs can be used and augmented effectively in section \ref{sec:LLM_used}.

Through advanced usage and augmentation techniques, LLMs can be deployed as so-called AI agents: artificial entities that sense their environment, make decisions, and take actions. Previous research has focused on developing agents for specific tasks and domains. The emergent abilities demonstrated by LLMs make it possible to build general-purpose AI agents based on LLMs. 
While LLMs are trained to produce responses in static settings, AI agents need to take actions to interact with dynamic environment. Therefore, LLM-based agents often need to augment LLMs to e.g., obtain updated information from external knowledge bases, verify whether a system action produces the expected result, and cope with when things do not go as expected, etc. We will discuss in detail LLM-based agents in Section \ref{sec:LLM_used}. 


\begin{figure*}
\begin{center}
    \includegraphics [scale=0.52] {img/structure_paper.pdf}
\end{center}
  \caption{The paper structure.}
\label{fig:paper_structure}
\end{figure*}


\subsection{Paper Structure}
In the rest of this paper,
Section \ref{sec:LLM_models} presents an overview of the current state of the art of LLMs, focusing on three LLM families: GPT, LLaMA and PaLM. We then review some of the other representative LLMs that don't belong to any of those three families.
Section \ref{sec:LLM_built} discusses how LLMs are built, starting from data cleaning and tokenization, to model pre-training, instruction tuning, and alignment.
Section \ref{sec:LLM_used} explains how LLMs are used, and augmented, covering prompt engineering, augmenting LLMs through external knowledge, using external tools, and LLM agents.
Sections \ref{sec:llm_datasets} and \ref{sec:llm_performance} review popular datasets and benchmarks for evaluating LLMs, and summarize the reported LLM evaluation results.
%Section \ref{sec:LLM_applications} reviews the applications of LLMs in several important domains.
Finally, we conclude the paper in Section \ref{sec:LLM_challenges} by summarizing the challenges and future research directions. 
We also provide an overview of some of the most popular tools and frameworks for LLM development, deployment, and improvement, in Appendix.





==> others/intro-old.tex <==
\section{Introduction}

%\textcolor{blue}{
%Dr. Gao: it would be great if you can write the main part of introduction section, providing a pre-LLM history of NLP, and how it led to the birth of LLMs, and how the LLM based models improved over the past few years and took over many areas of NLP applications, their potentials, etc.}

Language modeling is a long-standing research topic, dating back to Shannon's exploration of his  theory of information to human language where Shannon measures how well simple n-gram models did at predicting or compressing natural text. 

Thereafter, language modeling becomes fundamental to many natural language understanding and generation tasks, ranging from speech recognition, machine translation, to information retrieval.

The recent advance on large-scale neural language models, pretrained on Web-scale text corpora, significantly extends the capabilities of large language models (LLMs), such as in-context learning, and makes LLMs the basic building blocks for the development of general-purpose AI agents or AGI.

As the field of LLMs is fast moving, LLM researchers and practitioners find it challenging to figure out a right recipe to build LLM-power AI systems for their tasks. This paper presents a snapshot of the current state of the art of LLMs (Section 2), how LLMs are trained (Section 3), evaluated (Section 4), and augmented (Section 5), and utilized in real-world applications (Section6). We hope that this paper will prove a valuable and accessible resource for students, researchers and developers. 

In the rest of this section, we briefly review the history of language models.
\begin{itemize}
    \item SLM -- text as a sequence of tokens, LM as a traditional ML model, n-gram, MT vs. SR 
    \item NLM -- representation learning via deep learning -- open doors to fuse with other modalities, for the first time, we can estimate the similarity between Chinese and English, or even image and text.
    \item PLM -- encoding world knowledge -- PLM + Finetuning -- context aware representation. BERT for all NLP tasks.
    \item LLM -- in context learning via prompting -- change the way we build AI systems.
\end{itemize}


\subsection{ LLM Capabilities} \label{LLM_capabilities}
Figure \ref{fig:llm_capabalities} shows the different categories and respective tasks in each category for LLM capabilities. The categorization of these capabilities comes from the fact that each part is an essential task that large language model, based on the application should be able to perform in a good manner.

\begin{figure*}
\begin{center}
    \includegraphics [scale=0.8] {img/LLMCapabalities.pdf}
\end{center}
    \caption{LLM capabilities: Domain specific; Domain unspecific; Bias and fairness.}
    \label{fig:llm_capabalities}
\end{figure*}

\subsubsection{General}
Tasks or capabilities that are not specific to a certain domain and posses a general understanding or capability that can be applied to more than one specific domain are noted as domain unspecific ones.

\textbf{Code Generation}

Code generation or program synthesis is the task of automatically generating computer programs from higher-level requirements or natural language descriptions as input \cite{hendrycksapps2021}. In the wake of the power of LLMs on sequence modeling, they have been customized for code generation by appraoching programs as textual sequences \cite{zhang2023planning}. Some of the LLMs for Code Generation tools include CodeBERT \cite{feng2020codebert}, PyMT5 \cite{clement2020pymt5},Codex \cite{chen2021evaluating}, GPT-Neo \cite{Black2021GPTNeoLS},  GPT-J \cite{wang2021gpt}, CodeGen\cite{nijkamp2022codegen}, AlphaCode \cite{li2022competition}, InCoder \cite{fried2023incoder} and more.

\textbf{Reading Comprehension}

The Reading comprehension refers to the ability to comprehend written content, understand its meaning, and integrate it with what the reader already knows. Reading comprehension is based on two interconnected abilities: word reading and language comprehension \cite{rayner2001psychological}. In NLP domain,  the Machine Reading Comprehension or Reading Comprehension is a task designed to assess a machine's ability to read and grasp natural language by asking it to answer questions based on a given context \cite{liu2019neural}.

\textbf{Reasoning}

Reasoning refres to the cognitive process by which humans make sense of their circumstances. Reasoning is required to understand the experiences, draw conclusions from information, and convey new ideas \cite{leighton2004nature}.  Reasoning is a fundamental component in tasks such as problem solving, decision-making, and critical thinking \cite{huang2022towards}. Reasoning involves many different aspects such as arithmetic reasoning, symbolic, and commonsense reasoning. Each of these capabilities on its own brings additional value to the other capabilities as well.

\textbf{Text Summarization}

Text summarization involves distilling long documents with precise and coherent summaries while retaining the primary meaning and key information \cite{basyal2023text}. Summarization is one of the examples of the basic capabilities that LLMs can posses. Other tasks that are similar are noted as sentiment analysis, part of speech tagging, named entity recognition, etc.

\textbf{Machine Translation}

Machine translation refers to the automatic process by which a computer converts text from one language to another without the need for human interaction. Machine translation is one of the important capabilities in this scope because it is one of the tasks that shows how much a LLM can perform multilingual or cross-lingual tasks.


\textbf{Tool Utilization}

To figure out complicated tasks, LLMs often leverage the external tools. These tools can take various forms like API calls, Python functions, plugins, and more. This task is designed to assess how LLMs can benefit from tools \cite{wang2023mint, zhuang2023toolqa}. Tool utilization is important in cases where LLM is seen as an agent or part of a multi-agent environment where it is supposed to address certain tasks by using different tools available to it.

\textbf{Fact Verification}

With the rise of misinformation in the news and on social media, the role of fact-checking has gained prominence \cite{guo2022survey}. Fact-checking entails determining the veracity of a claim, where a claim is defined as a factual assertion under inquiry \cite{pan2021zero}.  In the realm of LLMs, fact-checking specifically assesses the truthfulness of a natural-language claim \cite{kadavath2022language}.

\subsubsection{Domain Specific}
Domain specific tasks or capabilities are those than are specific to a certain domain such as legal or medical. These capabilities can be considered as a very pin-pointed set of skills that aim to solve specific problems in specific domains. These capabilities can not be generalized to other domain but the learned task accomplishment can be generalized.

Large language models ...








==> others/intro.tex <==
\section{Introduction}

%\textcolor{blue}{
%Dr. Gao: it would be great if you can add more details about LLM applications as you shared over email with me before, scaling law, etc. in intro}


Language modeling is a long-standing research topic, dating back to Shannon's exploration of  information theory to human language where he measures how well simple n-gram language models predict or compress natural language text. 

Thereafter, statistical language modeling becomes fundamental to many natural language understanding and generation tasks, ranging from speech recognition, machine translation, to information retrieval \cite{jelinek1998statistical,manning1999foundations,manning2009introduction}.

The recent advance on large-scale neural language models, pretrained on Web-scale text corpora, significantly extends the capabilities of large language models (LLMs), such as in-context learning, making LLMs the basic building blocks for the development of general-purpose AI agents or AGI.

As the field of LLMs is fast moving, LLM researchers and practitioners find it challenging to figure out right recipes to build LLM-power AI systems for their tasks. This paper presents a snapshot of the current state of the art of LLMs (Section 2), how LLMs are built (Section 3), utilized (Section 4), evaluated (Section 5), and augmented (Section 6) for real-world applications (Section 7). We hope that this paper will prove a valuable and accessible resource for students, researchers and developers. 

In the rest of this section, we briefly review the history of language models (and the expansion of their abilities).
\begin{itemize}
    \item SLM -- text as a sequence of tokens, LM as a traditional ML model, n-gram for language understanding and generation, MT vs. SR 
    \item NLM -- representation learning via deep learning -- open doors to fuse with other modalities, for the first time, we can estimate the similarity between Chinese and English, or even image and text. LM for search.
    \item PLM -- encoding world knowledge -- PLM + Finetuning -- context aware representation. BERT for all NLP tasks.
    \item LLM -- in context learning via prompting -- change the way we build AI systems.
\end{itemize}
